Unsupervised Accelerated MRI Reconstruction via Ground-Truth-Free Flow Matching

Accelerated magnetic resonance imaging involves reconstructing fully sampled images from undersampled k-space measurements. Current state-of-the-art approaches have mainly focused on either end-to-end supervised training inspired by compressed sensing formulations, or posterior sampling methods built on modern generative models. However, their efficacy heavily relies on large datasets of fully sampled images, which may not always be available in practice. To address this issue, we propose an unsupervised MRI reconstruction method based on ground-truth-free flow matching (GTF$^2$M). Particularly, the GTF$^2$M learns a prior denoising process of fully sampled ground-truth images using only undersampled data. Based on that, an efficient cyclic reconstruction algorithm is further proposed to perform forward and backward integration in the dual space of image-space signal and k-space measurement. We compared our method with state-of-the-art learning-based baselines on the fastMRI database of both single-coil knee and multi-coil brain MRIs. The results show that our proposed unsupervised method can significantly outperform existing unsupervised approaches, and achieve performance comparable to most supervised end-to-end and prior learning baselines trained on fully sampled MRI, while offering greater efficiency than the compared generative model-based approaches.

==> 02_background.tex <==
\section{Background and Related Work}
\label{sec:background}

For MRI reconstruction as an inverse problem, the forward model is defined as $\bm{y}=\bm{Ax}+\bm{e}$, where $\bm{y}=(\bm{y}_c)_{c=1}^C\triangleq[\bm{y}_1^{\intercal},\dots,\bm{y}_C^{\intercal}]^{\intercal}\in\mathds{C}^{Cd}$ is the subsampled k-space measurement collected from $C$ coils, $\bm{x}\in\mathds{C}^D$ is the original image-space signal that we want to reconstruct, and noise $\bm{e}$ follows a complex Gaussian distribution $\mathcal{CN}(\bm{0},2\sigma^2\bm{I}_{Cd})$. 
The forward operator $\bm{A}$ takes the form
\begin{equation}\label{eq:forward_model}
  \bm{A} = \mqty[\dmat{\bm{MF},\ddots,\bm{MF}}]\mqty[\bm{S}_1\\\vdots\\\bm{S}_C],
\end{equation}
where $\bm{M}=\mqty[\bm{I}_d\mid\bm{0}]\bm{T}\in\mathds{R}^{d\times D}$ for some permutation matrix $\bm{T}\in\mathds{R}^{D\times D}$ represents the mask in k-space, $\bm{F}\in\mathds{C}^{D\times D}$ denotes the matrix of discrete Fourier transform, and $\bm{S}_c\in\mathds{C}^{D\times D}$ is a diagonal matrix encoding the sensitivity map of the $c$-th coil.

\subsection{Reconstruction as Unrolled Optimisation}
Conventionally, reconstruction of MRI is formulated as a variational problem solved with compressed sensing (CS) based methods \cite{journal/spm/lustig2008}.
Recently, MRI reconstruction has been formulated as a dealiasing problem via a learnt unrolled optimisation scheme \cite{journal/spm/knoll2020,journal/spm/liang2020,journal/mrm/hammernik2021}, namely
\begin{equation}
  \min_{\bm{\theta}}\min_{\bm{x}} \left\{\lambda \norm{\bm{Ax}-\bm{y}}_2^2 + \norm{\mathcal{R}_{\bm{\theta}}(\bm{x})}_2^2\right\},
\end{equation}
where $\mathcal{R}_{\bm{\theta}}(\cdot)$ is a regularisation term.
The inner optimisation problem can be solved using half quadratic splitting, unrolled as the alternating steps
\begin{subequations}
  \begin{align}
    \bm{z}_{i+1} &\triangleq\argmin_{\bm{z}}\left\{ \mathcal{R}_{\bm{\theta}}(\bm{z}) + \mu\norm{\bm{z}-\bm{x}_i}_2^2\right\} \label{eq:proximal} \\
    \bm{x}_{i+1} &\triangleq \argmin_{\bm{x}}\left\{ \gamma\norm{\bm{Ax}-\bm{y}}_2^2+\norm{\bm{x}-\bm{z}_{i+1}}_2^2\right\}, \label{eq:dc}
  \end{align}
\end{subequations}
for $i=0,\dots,K-1$, where $\gamma\triangleq\nicefrac{\lambda}{\mu}$ and the proximal operator \cref{eq:proximal} is often modelled implicitly by a residual network $\bm{z}_{i+1}\triangleq \bm{x}_i+\bm{h_{\theta}}(\bm{x}_i)$, while the data consistency step \cref{eq:dc} can be solved via proximal gradient descent \cite{journal/mrm/hammernik2018}, conjugate gradient \cite{journal/tmi/aggarwal2018}, or with closed-form solution for single-coil reconstruction \cite{journal/tmi/schlemper2017, journal/tmi/qin2019}.

\subsection{Flow Matching for Generative Modelling}\label{sec:flow_matching}
Flow matching is a recently proposed technique for generative modelling \cite{conference/iclr/liu2023,conference/iclr/lipman2023,conference/icml/esser2024}, which operates on a probability flow $p_t$ by progressively transforming a simple base distribution $p_1$ into a more complex target distribution $p_0$ of the observed data $\bm{x}\in\mathcal{X}\subset\mathds{R}^D$.
The transformation is defined by a diffeomorphic mapping $\phi_t:[0,1]\times\mathds{R}^D\rightarrow\mathds{R}^D$, which can be obtained with an ordinary differential equation (ODE) given a time-dependent vector field $\bm{u}_t:[0,1]\times\mathds{R}^D\rightarrow\mathds{R}^D$, 
\begin{equation}
  \bm{z}_t\triangleq\phi_t(\bm{z}_1),\quad \dd\bm{z}_t = \bm{u}_t(\bm{z}_t)\,\dd t, \quad\forall\,\bm{z}_1\sim p_1,
\end{equation}
with the boundary condition $\phi_1=\operatorname{id}$.
Then, the probability flow $p_t$ is computed using the push-forward (or change of variables) operator: $p_t=[\phi_t]_{\sharp}p_1$.
The base distribution $p_1$ usually follows a standard Gaussian, and thus $\phi_t(\cdot)$ can be viewed as a continuous denoising function with $\bm{u}_t(\cdot)$ its infinitesimal residual.

The marginal vector field $\bm{u}_t(\cdot)$ generating the probability flow can be constructed via the conditional path and vector field.
Specifically, given a sample $\bm{\epsilon}\sim p_1=\mathcal{N}(\bm{0},\bm{I}_D)$, we define the conditional path $\psi_t(\bm{\omega})$ and vector field $\bm{u}_{t\mid\bm{\omega}}(\cdot)$ where $\bm{\omega}\triangleq(\bm{x},\bm{\epsilon})$ as 
\begin{equation}
  \begin{aligned}
    \psi_t(\bm{\omega})&\triangleq a_t\bm{x}+b_t\bm{\epsilon}, \quad\forall\,\bm{\omega}\sim p_{\bm{\omega}}\in\mathcal{C}(p_0,p_1) \\ 
    \bm{u}_{t\mid\bm{\omega}}(\cdot)&\triangleq\psi_t'(\bm{\omega})=a_t'\bm{x}+b_t'\bm{\epsilon},\quad \forall\,t\in[0,1]
  \end{aligned}
\end{equation}
where $\mathcal{C}(\cdot,\cdot)$ denotes the coupling of two distributions, $\psi_t'\equiv\nicefrac{\dd\psi_t}{\dd t}$, $a_0=b_1=1$ and $a_1=b_0=0$.
One common instantiation is the independent coupling $p_{\bm{\omega}}=p_0\times p_1$ and linear interpolation $\psi_t(\bm{\omega})=(1-t)\bm{x}+t\bm{\epsilon}$ with $p_{t}(\cdot\mid\bm{\omega})=\delta_{(1-t)\bm{x}+t\bm{\epsilon}}(\cdot)$. 
Then, the marginal vector field $\bm{u}_t$ that generates $p_t$ can be constructed by 
\begin{equation}
  \bm{u}_t(\bm{z}_t) \triangleq\mathbb{E}_{\bm{\omega}\sim p_t(\cdot\mid\bm{z}_t)}\left[\bm{u}_{t\mid\bm{\omega}}(\bm{z}_t)\right]= \mathbb{E}_{\bm{\omega}\sim p_0\times p_1}\left[\bm{u}_{t\mid\bm{\omega}}(\bm{z}_t)\frac{p_t(\bm{z}_t\mid\bm{\omega})}{p_t(\bm{z}_t)}\right],
\end{equation}
where $p_t(\cdot)=\mathbb{E}_{\bm{\omega}\sim p_0\times p_1}[p_t(\cdot\mid\bm{\omega})]$, satisfying the continuity equation \cite{book/villani2009}.

Given the above probability flow defined with $\bm{u}_t(\cdot)$, flow matching learns the generative mapping between $p_1$ and $p_0$ by regressing the vector field using the objective $\min_{\bm{\theta}}\mathbb{E}_{t\sim p_T,\bm{z}_t\sim p_t(\cdot)}\norm{\bm{v_{\theta}}(\bm{z}_t,t)-\bm{u}_t(\bm{z}_t)}_2^2$,
which is found equivalent to the more tractable conditional flow matching objective:
\begin{equation}
  \min_{\bm{\theta}}\mathbb{E}_{t\sim p_T,\bm{\omega}\sim p_0\times p_1,\bm{z}_{t\mid\bm{\omega}}\sim p_t(\cdot\mid\bm{\omega})}\norm{\bm{v_{\theta}}(\bm{z}_{t\mid\bm{\omega}},t)-\bm{u}_{t\mid\bm{\omega}}(\bm{z}_{t\mid\bm{\omega}})}_2^2,
\end{equation}
where $\bm{z}_{t\mid\bm{\omega}}$ is sampled as $\bm{z}_{t\mid\bm{\omega}}\triangleq\psi_t(\bm{\omega})=a_t\bm{x}+b_t\bm{\epsilon}$.

\subsection{Generalised Stein's Unbiased Risk Estimator}
For a denoising problem, the measurement is observed from the forward model $\bm{y}=\bm{x}+\bm{e}$ with noise distribution $\bm{e}\sim\mathcal{N}(\bm{0},\sigma^2\bm{I}_D)$.
The Stein's unbiased risk estimator (SURE) \cite{journal/ans/stein1981} derives an unbiased estimate of the mean squared error (MSE) for a denoiser $\bm{h}(\bm{y})$ as
\begin{equation}
  \mathbb{E}_{\bm{x}}\norm{\bm{h}(\bm{y})-\bm{x}}_2^2 = 
  \mathbb{E}_{\bm{x}}\left[\norm{\bm{h}(\bm{y})-\bm{y}}_2^2 + 2\sigma^2\nabla_{\bm{y}}\cdot\bm{h}(\bm{y})\right] - D\sigma^2.
\end{equation}
The Generalised SURE (GSURE) \cite{journal/tsp/eldar2008} extends the framework to a general inverse problem $\bm{y}=\bm{Ax}+\bm{e}$ with a possibly rank-deficient forward operator $\bm{A}\in\mathds{R}^{d\times D}$ and the noise $\bm{e}\sim\mathcal{N}(\bm{0},\bm{C})$.
Then, an unbiased estimate of the projected MSE in the range space of $\bm{A}^{\intercal}$ is given by
\begin{equation}\label{eq:gsure}
  \begin{aligned}
    \mathbb{E}_{\bm{x}}\norm{\bm{P}(\bm{h}(\bm{y})-\bm{x})}_2^2 = \mathbb{E}_{\bm{x}}\left[\norm{\bm{P}(\bm{h}(\bm{\mu})-\widehat{\bm{x}}_{\text{ML}})}_2^2 
    + 2\nabla_{\bm{\mu}}\cdot\bm{P}\bm{h}(\bm{\mu})\right] + \operatorname{const.},
  \end{aligned}
\end{equation}
where $\bm{P}=\bm{A}^{\dag}\bm{A}$ is the projection operator, $\bm{\mu}=\bm{A}^{\intercal}\bm{C}^{-1}\bm{y}$ is a sufficient statistic for $\bm{x}$, $\bm{A}^{\dag}$ is the Moore-Penrose pseudo-inverse of $\bm{A}$, and $\widehat{\bm{x}}_{\text{ML}}=(\bm{A}^{\intercal}\bm{C}^{-1}\bm{A})^{\dag}\bm{C}^{-1}\bm{y}$ denotes the maximum likelihood estimate (MLE) of $\bm{x}$.
However, the GSURE estimate only considers the range-space MSE, ignoring the null-space component.
The ENsemble SURE (ENSURE) framework \cite{journal/tmi/aggarwal2022} resolves this issue by assuming randomness of the forward operator $\bm{A}$ and shows that the expectation of the weighted GSURE loss over the forward operator and the measurement is identical to the true MSE.
That is, if the forward operator $\bm{A}_s$ is indexed by some random variable $s\sim p(s)$, then by denoting $\bm{W}\triangleq\mathbb{E}_s[\bm{P}_s]^{-\nicefrac{1}{2}}$ and $\bm{R}_s\triangleq\bm{W}\bm{P}_s$, we have
\begin{equation}\label{eq:ensure}
  \mathbb{E}_{\bm{x},s}\norm{\bm{h}(\bm{y}_s)-\bm{x}}_2^2 = \mathbb{E}_{\bm{x},s}\norm{\bm{R}_s(\bm{h}(\bm{y}_s)-\bm{x})}_2^2.
\end{equation}
For single-coil reconstruction where $\bm{A}_s=\bm{M}_s\bm{F}$, the projection operator $\bm{R}_s$ has a closed-form expression as
$\bm{R}_s = \bm{F}^*\bm{T}_s^{\intercal}\operatorname{diag}(p_1^{-0.5},\dots,p_d
^{-0.5},0,\dots,0)\bm{T}_s\bm{F}$, where $p_i$ denotes the probability that the $i$-th k-space measurement is acquired.
